MQBench: Towards Reproducible and Deployable Model Quantization Benchmark

Model quantization has emerged as an indispensable technique to accelerate deep learning inference. While researchers continue to push the frontier of quantization algorithms, existing quantization work is often unreproducible and undeployable. This is because researchers do not choose consistent training pipelines and ignore the requirements for hardware deployments. In this work, we propose Model Quantization Benchmark (MQBench), a first attempt to evaluate, analyze, and benchmark the reproducibility and deployability for model quantization algorithms. We choose multiple different platforms for real-world deployments, including CPU, GPU, ASIC, DSP, and evaluate extensive state-of-the-art quantization algorithms under a unified training pipeline. MQBench acts like a bridge to connect the algorithm and the hardware. We conduct a comprehensive analysis and find considerable intuitive or counter-intuitive insights. By aligning the training settings, we find existing algorithms have about the same performance on the conventional academic track. While for the hardware-deployable quantization, there is a huge accuracy gap which remains unsettled. Surprisingly, no existing algorithm wins every challenge in MQBench, and we hope this work could inspire future research directions.

==> sections/2_related.tex <==
\section{Related Work}

\paragraph{Efficient Inference Techniques.} 
Improving the inference efficiency of deep neural networks on resource-constrained edge devices has recently drawn extensive attention. Starting from \cite{han2015learning,gong2014compressing,han2016deep,denton2014exploiting,vanhoucke2011improving}, one line of research focuses on compressing pre-trained neural networks, including i) network pruning that removes less-important units \cite{han2015learning,frankle2018the} or channels \cite{liu2017learning,he2017channel}; ii) network quantization that reduces the bitwidth of parameters \cite{han2016deep,courbariaux2015binaryconnect} or activations \cite{jacob2018quantization,wang2019haq}. However, these techniques cannot handle the training phase, as they rely on a well-trained model on the target task as the starting point. 

Another line of research focuses on lightweight neural architectures by either manual design \cite{iandola2016squeezenet,howard2017mobilenets,sandler2018mobilenetv2,zhang2018shufflenet,huang2018condensenet} or neural architecture search \cite{tan2018mnasnet,cai2019proxylessnas,wu2018fbnet,cai2018efficient}. 
These lightweight neural networks provide highly competitive accuracy \cite{tan2019efficientnet,cai2020once} while significantly improving inference efficiency.
However, concerning the training memory efficiency, key bottlenecks are not solved: \textbf{the training memory is dominated by activations, not parameters} (Figure~\ref{fig:memory_training_versus_inference}).

There are also some non-deep learning methods \cite{kumar2017resource,gupta2017protonn,edgeml03} that are designed for efficient inference on edge devices. These methods are suitable for handling simple tasks like MNIST. However, for more complicated tasks, we still need the representation capacity of deep neural networks.

\paragraph{Memory Footprint Reduction.} 
Researchers have been seeking ways to reduce the training memory footprint. One typical approach is to re-compute discarded activations during backward~\cite{gruslys2016memory,chen2016training}. This approach reduces memory usage at the cost of a large computation overhead. Thus it is not preferred for edge devices. Layer-wise training \cite{greff2016highway} can also reduce the memory footprint compared to end-to-end training. However, it cannot achieve the same level of accuracy as end-to-end training. Another representative approach is through activation pruning \cite{liu2019dynamic}, which builds a dynamic sparse computation graph to prune activations during training. Similarly, \cite{wang2018training} proposes to reduce the bitwidth of training activations by introducing new reduced-precision floating-point formats. Besides reducing the training memory cost, there are some techniques that focus on reducing the peak inference memory cost, such as RNNPool \cite{saha2020rnnpool} and MemNet \cite{liu2019memnet}.
Our method is orthogonal to these techniques and can be combined to further reduce the memory footprint. 

\paragraph{Transfer Learning.} 
Neural networks pre-trained on large-scale datasets (e.g., ImageNet \cite{deng2009imagenet}) are widely used as a fixed feature extractor for transfer learning, then only the last layer needs to be fine-tuned \cite{chatfield2014return,donahue2014decaf,gan2015devnet,sharif2014cnn}. 
This approach does not require to store the intermediate activations of the feature extractor, and thus is memory-efficient. However, the capacity of this approach is limited, resulting in poor accuracy, especially on datasets \cite{maji2013fine,krause20133d}  whose distribution is far from ImageNet (e.g., only 45.9\% Aircraft top1 accuracy achieved by Inception-V3 \cite{mudrakarta2018k}). Alternatively, fine-tuning the full network can achieve better accuracy \cite{kornblith2019better,cui2018large}. But it requires a vast memory footprint and hence is not friendly for training on edge devices. Recently, \cite{mudrakarta2019k,frankle2020training} propose to only update parameters of the batch normalization (BN) \cite{ioffe2015batch} layers, which greatly reduces the number of trainable parameters. \textbf{Unfortunately, parameter-efficiency doesn't translate to memory-efficiency.} It still requires a large amount of memory (e.g., 326MB under batch size 8) to store the input activations of the BN layers (Table~\ref{tab:transfer_results_under_different_backbones}). Additionally, the accuracy of this approach is still much worse than fine-tuning the full network (70.7\% v.s. 85.5\%; Table~\ref{tab:transfer_results_under_different_backbones}). People can also partially fine-tune some layers, but how many layers to select is still ad hoc. This paper provides a systematic approach to save memory without losing accuracy.

